IMEXnet: A Forward Stable Deep Neural Network

Deep convolutional neural networks have revolutionized many machine learning and computer vision tasks, however, some remaining key challenges limit their wider use. These challenges include improving the network's robustness to perturbations of the input image and the limited ``field of view'' of convolution operators. We introduce the IMEXnet that addresses these challenges by adapting semi-implicit methods for partial differential equations. Compared to similar explicit networks, such as residual networks, our network is more stable, which has recently shown to reduce the sensitivity to small changes in the input features and improve generalization. The addition of an implicit step connects all pixels in each channel of the image and therefore addresses the field of view problem while still being comparable to standard convolutions in terms of the number of parameters and computational complexity. We also present a new dataset for semantic segmentation and demonstrate the effectiveness of our architecture using the NYU Depth dataset.

==> img/example1/preamble.tex <==
\usepackage{amsmath,amsfonts,amssymb}
\usepackage{xcolor}
\usepackage{tikz}
\usetikzlibrary{arrows,calc}
\usepackage{relsize}
\usepackage{pgfplots}
%\usepackage{tgpagella}
%\usepackage{mathpazo}
\usepackage[scaled=.95]{helvet}
% \usepackage{courier}
% \usepackage[helvet]{sfmath}
\renewcommand{\familydefault}{\sfdefault}

\newdimen\iwidth
\newdimen\iheight

% \usepackage{siunitx}
% \sisetup{round-precision=4,round-mode=figures,scientific-notation=true}


==> img/figure5/convergence.tex <==
% This file was created by matlab2tikz.
% Minimal pgfplots version: 1.3
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%
\pgfplotsset{every tick label/.append style={font=\large}}
\begin{tikzpicture}

\begin{axis}[%
width=0.95092\iwidth,
height=\iheight,
at={(0\iwidth,0\iheight)},
scale only axis,
xmin=0,
xmax=500,
xlabel={epochs},
ymin=0,
ymax=1,
ylabel={training loss},
legend style={legend cell align=left,align=left,draw=white!15!black}
]
\addplot [color=mycolor1,solid,line width=3.0pt]
  table[row sep=crcr]{%
1	0.989\\
2	0.986\\
3	0.983\\
4	0.98\\
5	0.977\\
6	0.973\\
7	0.97\\
8	0.967\\
9	0.963\\
10	0.96\\
11	0.956\\
12	0.953\\
13	0.949\\
14	0.945\\
15	0.942\\
16	0.938\\
17	0.934\\
18	0.93\\
19	0.926\\
20	0.922\\
21	0.917\\
22	0.913\\
23	0.908\\
24	0.904\\
25	0.899\\
26	0.894\\
27	0.889\\
28	0.884\\
29	0.879\\
30	0.874\\
31	0.869\\
32	0.863\\
33	0.858\\
34	0.852\\
35	0.846\\
36	0.84\\
37	0.834\\
38	0.828\\
39	0.821\\
40	0.815\\
41	0.808\\
42	0.801\\
43	0.794\\
44	0.787\\
45	0.779\\
46	0.772\\
47	0.764\\
48	0.756\\
49	0.748\\
50	0.74\\
51	0.731\\
52	0.723\\
53	0.714\\
54	0.705\\
55	0.696\\
56	0.686\\
57	0.676\\
58	0.667\\
59	0.657\\
60	0.647\\
61	0.636\\
62	0.626\\
63	0.615\\
64	0.604\\
65	0.593\\
66	0.582\\
67	0.571\\
68	0.56\\
69	0.548\\
70	0.537\\
71	0.525\\
72	0.513\\
73	0.502\\
74	0.49\\
75	0.478\\
76	0.466\\
77	0.455\\
78	0.443\\
79	0.432\\
80	0.42\\
81	0.409\\
82	0.397\\
83	0.386\\
84	0.375\\
85	0.364\\
86	0.354\\
87	0.343\\
88	0.333\\
89	0.323\\
90	0.314\\
91	0.304\\
92	0.295\\
93	0.286\\
94	0.278\\
95	0.27\\
96	0.262\\
97	0.254\\
98	0.247\\
99	0.24\\
100	0.234\\
101	0.227\\
102	0.221\\
103	0.216\\
104	0.21\\
105	0.205\\
106	0.201\\
107	0.196\\
108	0.192\\
109	0.188\\
110	0.184\\
111	0.181\\
112	0.177\\
113	0.174\\
114	0.171\\
115	0.169\\
116	0.166\\
117	0.164\\
118	0.162\\
119	0.16\\
120	0.158\\
121	0.156\\
122	0.155\\
123	0.153\\
124	0.152\\
125	0.15\\
126	0.149\\
127	0.148\\
128	0.147\\
129	0.146\\
130	0.145\\
131	0.144\\
132	0.143\\
133	0.143\\
134	0.142\\
135	0.141\\
136	0.141\\
137	0.14\\
138	0.14\\
139	0.139\\
140	0.138\\
141	0.138\\
142	0.138\\
143	0.137\\
144	0.137\\
145	0.136\\
146	0.136\\
147	0.136\\
148	0.135\\
149	0.135\\
150	0.135\\
151	0.134\\
152	0.134\\
153	0.134\\
154	0.133\\
155	0.133\\
156	0.133\\
157	0.132\\
158	0.132\\
159	0.132\\
160	0.132\\
161	0.131\\
162	0.131\\
163	0.131\\
164	0.131\\
165	0.131\\
166	0.13\\
167	0.13\\
168	0.13\\
169	0.13\\
170	0.13\\
171	0.129\\
172	0.129\\
173	0.129\\
174	0.129\\
175	0.129\\
176	0.128\\
177	0.128\\
178	0.128\\
179	0.128\\
180	0.128\\
181	0.127\\
182	0.127\\
183	0.127\\
184	0.127\\
185	0.127\\
186	0.127\\
187	0.126\\
188	0.126\\
189	0.126\\
190	0.126\\
191	0.126\\
192	0.126\\
193	0.126\\
194	0.125\\
195	0.125\\
196	0.125\\
197	0.125\\
198	0.125\\
199	0.125\\
200	0.125\\
201	0.124\\
202	0.124\\
203	0.124\\
204	0.124\\
205	0.124\\
206	0.124\\
207	0.124\\
208	0.124\\
209	0.123\\
210	0.123\\
211	0.123\\
212	0.123\\
213	0.123\\
214	0.123\\
215	0.123\\
216	0.123\\
217	0.123\\
218	0.122\\
219	0.122\\
220	0.122\\
221	0.122\\
222	0.122\\
223	0.122\\
224	0.122\\
225	0.122\\
226	0.122\\
227	0.121\\
228	0.121\\
229	0.121\\
230	0.121\\
231	0.121\\
232	0.121\\
233	0.121\\
234	0.121\\
235	0.121\\
236	0.121\\
237	0.121\\
238	0.12\\
239	0.12\\
240	0.12\\
241	0.12\\
242	0.12\\
243	0.12\\
244	0.12\\
245	0.12\\
246	0.12\\
247	0.12\\
248	0.119\\
249	0.119\\
250	0.119\\
251	0.119\\
252	0.119\\
253	0.119\\
254	0.119\\
255	0.119\\
256	0.119\\
257	0.119\\
258	0.119\\
259	0.119\\
260	0.118\\
261	0.118\\
262	0.118\\
263	0.118\\
264	0.118\\
265	0.118\\
266	0.118\\
267	0.118\\
268	0.118\\
269	0.118\\
270	0.118\\
271	0.118\\
272	0.118\\
273	0.117\\
274	0.117\\
275	0.117\\
276	0.117\\
277	0.117\\
278	0.117\\
279	0.117\\
280	0.117\\
281	0.117\\
282	0.117\\
283	0.117\\
284	0.117\\
285	0.117\\
286	0.117\\
287	0.116\\
288	0.116\\
289	0.116\\
290	0.116\\
291	0.116\\
292	0.116\\
293	0.116\\
294	0.116\\
295	0.116\\
296	0.116\\
297	0.116\\
298	0.116\\
299	0.116\\
300	0.116\\
301	0.116\\
302	0.115\\
303	0.115\\
304	0.115\\
305	0.115\\
306	0.115\\
307	0.115\\
308	0.115\\
309	0.115\\
310	0.115\\
311	0.115\\
312	0.115\\
313	0.115\\
314	0.115\\
315	0.115\\
316	0.115\\
317	0.115\\
318	0.115\\
319	0.114\\
320	0.114\\
321	0.114\\
322	0.114\\
323	0.114\\
324	0.114\\
325	0.114\\
326	0.114\\
327	0.114\\
328	0.114\\
329	0.114\\
330	0.114\\
331	0.114\\
332	0.114\\
333	0.114\\
334	0.114\\
335	0.114\\
336	0.114\\
337	0.113\\
338	0.113\\
339	0.113\\
340	0.113\\
341	0.113\\
342	0.113\\
343	0.113\\
344	0.113\\
345	0.113\\
346	0.113\\
347	0.113\\
348	0.113\\
349	0.113\\
350	0.113\\
351	0.113\\
352	0.113\\
353	0.113\\
354	0.113\\
355	0.113\\
356	0.112\\
357	0.112\\
358	0.112\\
359	0.112\\
360	0.112\\
361	0.112\\
362	0.112\\
363	0.112\\
364	0.112\\
365	0.112\\
366	0.112\\
367	0.112\\
368	0.112\\
369	0.112\\
370	0.112\\
371	0.112\\
372	0.112\\
373	0.112\\
374	0.112\\
375	0.112\\
376	0.111\\
377	0.111\\
378	0.111\\
379	0.111\\
380	0.111\\
381	0.111\\
382	0.111\\
383	0.111\\
384	0.111\\
385	0.111\\
386	0.111\\
387	0.111\\
388	0.111\\
389	0.111\\
390	0.111\\
391	0.111\\
392	0.111\\
393	0.111\\
394	0.111\\
395	0.111\\
396	0.111\\
397	0.111\\
398	0.11\\
399	0.11\\
400	0.11\\
401	0.11\\
402	0.11\\
403	0.11\\
404	0.11\\
405	0.11\\
406	0.11\\
407	0.11\\
408	0.11\\
409	0.11\\
410	0.11\\
411	0.11\\
412	0.11\\
413	0.11\\
414	0.11\\
415	0.11\\
416	0.11\\
417	0.11\\
418	0.11\\
419	0.11\\
420	0.11\\
421	0.109\\
422	0.109\\
423	0.109\\
424	0.109\\
425	0.109\\
426	0.109\\
427	0.109\\
428	0.109\\
429	0.109\\
430	0.109\\
431	0.109\\
432	0.109\\
433	0.109\\
434	0.109\\
435	0.109\\
436	0.109\\
437	0.109\\
438	0.109\\
439	0.109\\
440	0.109\\
441	0.109\\
442	0.109\\
443	0.109\\
444	0.109\\
445	0.108\\
446	0.108\\
447	0.108\\
448	0.108\\
449	0.108\\
450	0.108\\
451	0.108\\
452	0.108\\
453	0.108\\
454	0.108\\
455	0.108\\
456	0.108\\
457	0.108\\
458	0.108\\
459	0.108\\
460	0.108\\
461	0.108\\
462	0.108\\
463	0.108\\
464	0.108\\
465	0.108\\
466	0.108\\
467	0.108\\
468	0.108\\
469	0.108\\
470	0.107\\
471	0.107\\
472	0.107\\
473	0.107\\
474	0.107\\
475	0.107\\
476	0.107\\
477	0.107\\
478	0.107\\
479	0.107\\
480	0.107\\
481	0.107\\
482	0.107\\
483	0.107\\
484	0.107\\
485	0.107\\
486	0.107\\
487	0.107\\
488	0.107\\
489	0.107\\
490	0.107\\
491	0.107\\
492	0.107\\
493	0.107\\
494	0.107\\
495	0.107\\
};
\addlegendentry{ResNet};

\addplot [color=mycolor2,solid,line width=3.0pt]
  table[row sep=crcr]{%
1	0.917\\
2	0.912\\
3	0.907\\
4	0.902\\
5	0.897\\
6	0.892\\
7	0.887\\
8	0.881\\
9	0.876\\
10	0.871\\
11	0.865\\
12	0.859\\
13	0.854\\
14	0.848\\
15	0.842\\
16	0.835\\
17	0.829\\
18	0.823\\
19	0.816\\
20	0.809\\
21	0.803\\
22	0.796\\
23	0.789\\
24	0.782\\
25	0.774\\
26	0.767\\
27	0.759\\
28	0.751\\
29	0.743\\
30	0.735\\
31	0.726\\
32	0.718\\
33	0.709\\
34	0.7\\
35	0.691\\
36	0.682\\
37	0.672\\
38	0.662\\
39	0.652\\
40	0.642\\
41	0.631\\
42	0.621\\
43	0.61\\
44	0.599\\
45	0.588\\
46	0.577\\
47	0.565\\
48	0.553\\
49	0.541\\
50	0.53\\
51	0.518\\
52	0.507\\
53	0.493\\
54	0.481\\
55	0.469\\
56	0.457\\
57	0.443\\
58	0.43\\
59	0.418\\
60	0.405\\
61	0.394\\
62	0.383\\
63	0.368\\
64	0.356\\
65	0.344\\
66	0.331\\
67	0.32\\
68	0.309\\
69	0.296\\
70	0.286\\
71	0.275\\
72	0.265\\
73	0.253\\
74	0.244\\
75	0.233\\
76	0.225\\
77	0.215\\
78	0.207\\
79	0.198\\
80	0.191\\
81	0.182\\
82	0.175\\
83	0.168\\
84	0.162\\
85	0.155\\
86	0.15\\
87	0.145\\
88	0.141\\
89	0.136\\
90	0.13\\
91	0.126\\
92	0.123\\
93	0.12\\
94	0.116\\
95	0.114\\
96	0.11\\
97	0.108\\
98	0.104\\
99	0.103\\
100	0.099\\
101	0.098\\
102	0.097\\
103	0.095\\
104	0.094\\
105	0.091\\
106	0.09\\
107	0.089\\
108	0.087\\
109	0.086\\
110	0.086\\
111	0.085\\
112	0.083\\
113	0.082\\
114	0.083\\
115	0.082\\
116	0.081\\
117	0.08\\
118	0.079\\
119	0.079\\
120	0.084\\
121	0.079\\
122	0.077\\
123	0.077\\
124	0.078\\
125	0.085\\
126	0.077\\
127	0.076\\
128	0.075\\
129	0.075\\
130	0.074\\
131	0.074\\
132	0.074\\
133	0.073\\
134	0.073\\
135	0.073\\
136	0.073\\
137	0.072\\
138	0.072\\
139	0.072\\
140	0.071\\
141	0.072\\
142	0.071\\
143	0.073\\
144	0.078\\
145	0.071\\
146	0.07\\
147	0.07\\
148	0.069\\
149	0.069\\
150	0.069\\
151	0.069\\
152	0.068\\
153	0.068\\
154	0.068\\
155	0.068\\
156	0.068\\
157	0.067\\
158	0.067\\
159	0.067\\
160	0.067\\
161	0.067\\
162	0.066\\
163	0.066\\
164	0.066\\
165	0.066\\
166	0.066\\
167	0.066\\
168	0.066\\
169	0.065\\
170	0.065\\
171	0.065\\
172	0.065\\
173	0.065\\
174	0.064\\
175	0.064\\
176	0.064\\
177	0.064\\
178	0.064\\
179	0.064\\
180	0.063\\
181	0.063\\
182	0.063\\
183	0.063\\
184	0.063\\
185	0.064\\
186	0.069\\
187	0.064\\
188	0.063\\
189	0.062\\
190	0.063\\
191	0.062\\
192	0.062\\
193	0.062\\
194	0.061\\
195	0.061\\
196	0.062\\
197	0.061\\
198	0.061\\
199	0.061\\
200	0.061\\
201	0.061\\
202	0.061\\
203	0.061\\
204	0.06\\
205	0.06\\
206	0.06\\
207	0.06\\
208	0.061\\
209	0.06\\
210	0.06\\
211	0.059\\
212	0.059\\
213	0.059\\
214	0.059\\
215	0.059\\
216	0.061\\
217	0.059\\
218	0.06\\
219	0.059\\
220	0.059\\
221	0.059\\
222	0.06\\
223	0.059\\
224	0.06\\
225	0.059\\
226	0.06\\
227	0.06\\
228	0.058\\
229	0.058\\
230	0.058\\
231	0.058\\
232	0.057\\
233	0.057\\
234	0.057\\
235	0.057\\
236	0.057\\
237	0.057\\
238	0.057\\
239	0.057\\
240	0.057\\
241	0.057\\
242	0.057\\
243	0.057\\
244	0.056\\
245	0.057\\
246	0.056\\
247	0.057\\
248	0.056\\
249	0.056\\
250	0.056\\
251	0.056\\
252	0.056\\
253	0.056\\
254	0.056\\
255	0.056\\
256	0.055\\
257	0.055\\
258	0.055\\
259	0.055\\
260	0.055\\
261	0.055\\
262	0.055\\
263	0.055\\
264	0.055\\
265	0.055\\
266	0.055\\
267	0.054\\
268	0.054\\
269	0.054\\
270	0.054\\
271	0.054\\
272	0.054\\
273	0.054\\
274	0.054\\
275	0.054\\
276	0.054\\
277	0.054\\
278	0.054\\
279	0.053\\
280	0.053\\
281	0.053\\
282	0.053\\
283	0.053\\
284	0.053\\
285	0.053\\
286	0.053\\
287	0.053\\
288	0.053\\
289	0.053\\
290	0.053\\
291	0.052\\
292	0.052\\
293	0.052\\
294	0.052\\
295	0.052\\
296	0.052\\
297	0.052\\
298	0.052\\
299	0.052\\
300	0.052\\
301	0.052\\
302	0.052\\
303	0.051\\
304	0.052\\
305	0.051\\
306	0.051\\
307	0.051\\
308	0.051\\
309	0.051\\
310	0.051\\
311	0.051\\
312	0.051\\
313	0.051\\
314	0.051\\
315	0.051\\
316	0.051\\
317	0.05\\
318	0.051\\
319	0.05\\
320	0.05\\
321	0.05\\
322	0.05\\
323	0.05\\
324	0.05\\
325	0.05\\
326	0.05\\
327	0.049\\
328	0.05\\
329	0.049\\
330	0.05\\
331	0.049\\
332	0.049\\
333	0.049\\
334	0.049\\
335	0.049\\
336	0.049\\
337	0.049\\
338	0.049\\
339	0.049\\
340	0.049\\
341	0.049\\
342	0.049\\
343	0.048\\
344	0.049\\
345	0.048\\
346	0.048\\
347	0.048\\
348	0.048\\
349	0.048\\
350	0.048\\
351	0.048\\
352	0.048\\
353	0.048\\
354	0.048\\
355	0.048\\
356	0.048\\
357	0.047\\
358	0.048\\
359	0.047\\
360	0.047\\
361	0.047\\
362	0.047\\
363	0.047\\
364	0.047\\
365	0.048\\
366	0.047\\
367	0.046\\
368	0.046\\
369	0.046\\
370	0.046\\
371	0.046\\
372	0.046\\
373	0.047\\
374	0.047\\
375	0.047\\
376	0.047\\
377	0.047\\
378	0.046\\
379	0.046\\
380	0.045\\
381	0.046\\
382	0.046\\
383	0.047\\
384	0.045\\
385	0.046\\
386	0.045\\
387	0.046\\
388	0.045\\
389	0.045\\
390	0.045\\
391	0.045\\
392	0.046\\
393	0.046\\
394	0.047\\
395	0.045\\
396	0.045\\
397	0.045\\
398	0.045\\
399	0.044\\
400	0.044\\
401	0.044\\
402	0.045\\
403	0.045\\
404	0.044\\
405	0.045\\
406	0.044\\
407	0.044\\
408	0.044\\
409	0.044\\
410	0.044\\
411	0.044\\
412	0.044\\
413	0.043\\
414	0.044\\
415	0.043\\
416	0.044\\
417	0.043\\
418	0.044\\
419	0.043\\
420	0.043\\
421	0.045\\
422	0.044\\
423	0.043\\
424	0.045\\
425	0.044\\
426	0.043\\
427	0.043\\
428	0.043\\
429	0.042\\
430	0.042\\
431	0.043\\
432	0.042\\
433	0.043\\
434	0.042\\
435	0.042\\
436	0.042\\
437	0.043\\
438	0.042\\
439	0.042\\
440	0.042\\
441	0.043\\
442	0.042\\
443	0.042\\
444	0.042\\
445	0.041\\
446	0.042\\
447	0.041\\
448	0.041\\
449	0.042\\
450	0.042\\
451	0.042\\
452	0.041\\
453	0.041\\
454	0.041\\
455	0.041\\
456	0.042\\
457	0.042\\
458	0.041\\
459	0.041\\
460	0.042\\
461	0.041\\
462	0.041\\
463	0.041\\
464	0.041\\
465	0.04\\
466	0.041\\
467	0.042\\
468	0.04\\
469	0.04\\
470	0.041\\
471	0.04\\
472	0.04\\
473	0.041\\
474	0.041\\
475	0.04\\
476	0.04\\
477	0.04\\
478	0.041\\
479	0.04\\
480	0.042\\
481	0.041\\
482	0.04\\
483	0.04\\
484	0.04\\
485	0.039\\
486	0.04\\
487	0.039\\
488	0.04\\
489	0.039\\
490	0.039\\
491	0.039\\
492	0.039\\
493	0.04\\
494	0.039\\
495	0.04\\
};
\addlegendentry{IMEXnet};

\end{axis}
\end{tikzpicture}%

==> img/figure5/preamble.tex <==
\usepackage{amsmath,amsfonts,amssymb}
\usepackage{xcolor}
\usepackage{tikz}
\usetikzlibrary{arrows,calc}
\usepackage{relsize}
\usepackage{pgfplots}
%\usepackage{tgpagella}
%\usepackage{mathpazo}
\usepackage[scaled=.95]{helvet}
% \usepackage{courier}
% \usepackage[helvet]{sfmath}
\renewcommand{\familydefault}{\sfdefault}

\newdimen\iwidth
\newdimen\iheight

% \usepackage{siunitx}
% \sisetup{round-precision=4,round-mode=figures,scientific-notation=true}

